ElasTraS: An Elastic Transactional Data Store in the Cloud

Over the last couple of years, "Cloud Computing" or "Elastic Computing" has emerged as a compelling and successful paradigm for internet scale computing. One of the major contributing factors to this success is the elasticity of resources. In spite of the elasticity provided by the infrastructure and the scalable design of the applications, the elephant (or the underlying database), which drives most of these web-based applications, is not very elastic and scalable, and hence limits scalability. In this paper, we propose ElasTraS which addresses this issue of scalability and elasticity of the data store in a cloud computing environment to leverage from the elastic nature of the underlying infrastructure, while providing scalable transactional data access. This paper aims at providing the design of a system in progress, highlighting the major design choices, analyzing the different guarantees provided by the system, and identifying several important challenges for the research community striving for computing in the cloud.

==> aws.tex <==
\section{Amazon Web Services}
\label{sec:aws}
Since its launch about 2--3 years back, Amazon Web Services (AWS) has been extremely successful, and this is evident from the increasing number of their customers and their soaring revenues. When launched initially, the AWS suite only included basic services: the \emph{Elastic Compute Cloud (EC2)}, \emph{Simple Storage Service (S3)}, and \emph{Simple Queueing Service (SQS)}. But during the course of the past couple of services, a large number of additional services have been added to the AWS suite, which includes \emph{Amazon SimpleDB}, \emph{Elastic Block Storage (EBS)}, and \emph{Amazon CloudFront} (for content caching and delivery along the same lines of Akamai (\url{http://www.akamai.com/})) to name a few. In this section, we summarize the various aspects and features of the suite of services offered by AWS, with the goal of providing the readers the necessary background, before we dive into the technical details of the design of the system.

\subsection{Elastic Compute Cloud (EC2)}
\label{sec:ec2}

Amazon Elastic Compute Cloud (\url{http://aws.amazon.com/ec2/}) is a web-service which provides resizable compute capacity on demand where the users are charged for the amount of resources they consume. With machine instances capable of booting up within a few minutes, EC2 provides an excellent platform for deployment of scalable internet services and is designed to make scaling much easier and faster. Originally launched with only a few instance types and regions, the EC2 service has now expanded to supporting various hardware types (with varying amounts of processing, memory, and storage), various operating systems (including Linux and Windows based instances), as well as various geographic regions as well (US and Europe, with finer levels of granularity inside US). Priced at an affordable \$0.10 to \$0.80 (depending on the capability of the instances and associated resources) per hours usage, EC2 provides the applications large amount of compute power for relatively low cost. For example, running a \emph{Small Instance} (1 EC2 Compute Unit equivalent to a 1.0GHz Opteron or Xeon processor, 1.7GB memory, 160 GB of local storage) charged at \$0.10 per hour for one entire month incurs a cost of only \$72. The instances can be configured using specific operating systems, applications, libraries, etc., and the configuration can be saved as Amazon Machine Images (AMI) from which the instances can be booted up. In addition, data transfer between different AWS components in the same \emph{Availability Zones}~\footnote{\emph{Availability Zones} are distinct locations that are engineered to be insulated from failures in other availability zones.}, while support for \emph{Elastic IP Addresses}~\footnote{\emph{Elastic IP Addresses} are static IP addresses assigned to AWS accounts and can be used to route traffic internally to the appropriate physical instance.}, and mountable fault-tolerant storage (EBS which will be discussed later) allows greater flexibility to the developers to design and deploy scalable applications. Recently, EC2 came out of the beta phase, and Amazon's SLA for EC2 guarantee an availability of 99.95\% for each EC2 \emph{Region} (a \emph{Region} is a collection of \emph{Availability Zones}, examples of which include the US \emph{Region}), thereby allowing high availability is the application design is fault-tolerant. In addition to providing on-demand compute resources, for meeting the demands of the customers who have a predictable usage pattern, Amazon has recently (as of 03/12/2009) introduced \emph{EC2 Reserved Instances} which allows users with predictable usage patterns to further reduce costs by paying an upfront cost, and thereby incurring considerably less charge for the instance hours, while still allowing access to on-demand resources. In summary, with EC2, AWS provides the developers an entire selection of compute resources suiting various application and workload characteristics.

\subsection{Simple Storage Service (S3)}
\label{sec:s3}

Amazon's Simple Storage Service (\url{http://aws.amazon.com/s3/}), often referred to as the storage for the Internet, is web-service that allows the storage and retrieval of huge amount of data from anywhere on the web (including from other AWS services) while guaranteeing reliability, high throughput, and high availability. Data objects can range from 1 byte to 5GB and an unlimited number of objects can be stored. Each data object is contained in a bucket, and can be accessed by a URI. Users can create, read, update, or delete data objects remotely using a SOAP or REST-based interface. In addition, each S3 object can have an associated user-defined metadata (up to 4KB) which can be accessed and modified independent of the actual data object. S3 is designed to provide scalable access to data, and the individual throughput and response times are not affected by concurrent accesses. Amazon's SLA commits a monthly uptime percentage of at least 99.9\% during a monthly billing cycle, thereby providing an effective means of highly available storage for a huge amount of data. The fault-tolerance in S3 is provided through replication on multiple locations possibly distributed across multiple data centers. Therefore, to support high rad and write availability, replication must be done asynchronous to the updates. As a result, Amazon does not provide strong consistency guarantees, and the application must be cognizant of this fact. Again, users of S3 pay for whatever resources they use, and is also very affordably priced at about \$0.15 per GB per month, about \$0.15 per GB of data transferred to/from the internet, and \$0.01 per 1000 \texttt{PUT, COPY, POST,} and \texttt{LIST} requests and \$0.01 per 10,000 \texttt{GET} and other requests.

\subsection{Simple Queuing Service (SQS)}
\label{sec:sqs}

Amazon Simple Queue Service (\url{http://aws.amazon.com/sqs/}) provides a reliable, highly scalable, hosted queue for efficient storage of messages being transferred between computers, and has been designed with the goal to ease building of automated workflows. An application can create unlimited number of SQS queues, each of which can contain unlimited number of messages limited to 8KB of text in any format. This queue is designed for communicating small amount of information across machines, while bulk transfer can be achieved using S3. When a message is read by some process, then it is marked as ``locked'' and is not returned by subsequent calls within a specific time interval. This prevents simultaneous processing of the same message, and if the process reading a message does not delete it, then the ``lock'' is released and the message becomes available again. SQS exposes both a SOAP based and Query interfaces to the developers, and any computer on the internet can add or read messages. Again, SQS is priced affordably at \$0.01 per 10,000 SQS requests and data transfer rates are similar to that of S3. SQS does not guarantee FIFO access to the messages in the queues, but SQS provides at least once delivery of messages in the queues, but due to failures, a message might be delivered multiple times and a deleted message can also be delivered again. So, even though the queues are a reliable means of message transfer, but the applications must be cognizant about this.

\subsection{Amazon SimpleDB}
\label{sec:simpledb}

Amazon SimpleDB (\url{http://aws.amazon.com/simpledb/}) is a web-service that provides core data storage functionality of data indexing and querying. It can be viewed as a schema free \emph{key-value} store that automatically indexes the data and provides simple API for storage and access. It allows organization for structured data into domains and run queries on data contained in a domain. SimpleDB exposes an interface for querying the data using both API calls as well as SQL like syntax, while providing some simple aggregation operators. In order to keep the response times low, SimpleDB limits query execution time to 5 seconds. If a query is not complete within 5 seconds, SimpleDB will return the partial results computed, and would also return a handle which will allow the query to be re-computed from the point to which it was completed in the previous attempt. This is a scalable service for data management, and the cost incurred depends on the data stored, bandwidth transferred, and computation spent in answering the queries. Prices are comparable to other Amazon's services, with computation charged at \$0.14 per hour, and data transfer and storage rates similar to that of S3.

Even though Simple DB is referred to as a database, but its goals, functionality, as well as guarantees are considerably different from that of a traditional database. SimpleDB can be viewed more as a \emph{key-value} store that where there is a structure for the \emph{values} associated with the keys. Furthermore, SimpleDB does not provide any transactional guarantees on multiple keys, and all updates are best-effort, and concurrent updates to the same key might result in \emph{lost updates}. But SimpleDB has been designed with a goal which is different to that of traditional databases, and hence comparing it with a database would not be fair, both in terms of functionality as well as performance. Therefore, even though Amazon's solution for data management is capable of storing and querying huge amount of data, but it stops short of functionality of the database in terms of transactions and recovery.

\subsection{Elastic Block Storage (EBS)}
\label{sec:ebs}

Amazon Elastic Block Storage (\url{http://aws.amazon.com/ebs/}) is a service that provides block level storage volumes that can be mounted with EC2 instances just like normal disk volumes. EBS volumes are generally not physically collocated with the EC2 instances, and these volumes persist independent of the life of an instance. Therefore, EBS provides a means for highly available, highly reliable storage volumes that can be attached to a running EC2 instance and can be treated as a disk volume that is part of the instance. It allows creation of 1GB to 1TB volumes that are placed in a specific \emph{Availability Zone (AZ)}, and can be attached to EC2 instances in the same zone. A single instance can mount a number of volumes, allowing for higher disk throughput, while a single volume can only be attached to one instance at a given instant of time. The EBS instances are automatically replicated within the same AZ and are therefore tolerant to single hardware failures. It also supports point-in-time snapshots to be persisted to S3 for longer durability, and spawning copies of the EBS volume in a different AZ. Similar to other AWS services, the pricing of EBS is also very affordable, charging only \$0.10 per GB-month of provisioned storage, and \$0.10 per million I/O requests. For example, for running a medium web-server with about 100GB of data, and incurring on a average 100 I/O requests per second will incur a cost of \$26 for an entire month's operation (\$10 for storage and \$16 for I/O). Therefore, at a marginal cost of operation, EBS guarantees an annual failure of 0.1--0.5\% which is considerably lower compared to that of commodity disks which is around 4\%. In addition, the EBS volumes are designed to have better latency response compared to the storage provided along with the instances.

\subsection{Amazon CloudFront}
\label{sec:cloudfront}

Amazon CloudFront is a web-service for providing content delivery and act like a cache for bandwidth intensive mostly read-only content. This is the same model as Akamai, and is intended to work with other AWS services, providing the developers an easy way to distribute theore content to the end users, while guaranteeing low latency and high data transfer speeds. CloudFront delivers content through a network of edge locations with a mechanism of routing requests to the nearest edge location. The original content is stored in S3, and are cached in CloudFront on-demand, but CloudFront does not provide any guarantees on how long the content will be cached in the edge locations. The edge locations are spread across the globe, and the cost of using this service is very much comparable to the rates of S3.

\subsection{Amazon Elastic MapReduce}
\label{sec:mapreduce}

\subsection{Summary}
\label{sec:aws_summary}

In this section, we provided a summary of the various components of the suite of services supported by AWS. These include raw compute power (EC2), raw storage (S3), fault-tolerant disk volumes (EBS), efficient means of communication between distributed processes (SQS), and other higher level abstractions for structured data storage (SimpleDB) and content delivery (CloudFront). In summary, AWS provides the entire package that is needed for web-scale application development and deployment, with high scalability and availability. The only component missing in this entire suite of services is a scalable transactional data store which would allow database driven applications to scale seamlessly as well. And in this paper, we propose \elastras, with a target to fill this void.












==> conclusion.tex <==
\section{Discussion and Conclusion}
\label{sec:conclusion}

%In the two previous sections, we discuss the design and implementation sketch of \elastras. In this section, we discuss the various workloads that can be supported by \elastras, and the impact of the workload on the performance and scalability of the system, and the cost of its operations. %During this discussion, we identify a number of research challenges that need to be addressed for efficient performance of the system.

%\subsection{Transactional Workload in \elastras}
%\noindent \textit{A. Transactional Workload in \elastras}

The proposed design of \elastras\ can provide ACID guarantees for transactions that are limited to a single partition. Practice has shown that most web workloads are limited to single object accesses~\cite{vogels07_keynote,dynamo}, and hence, these transactional accesses can be trivially supported by \elastras. In addition, most enterprise systems are designed for statically partitioned databases, and transactions are limited to a single database partition, and \elastras\ can provide efficient, scalable, and elastic transactional access to the partitioned data store. In such a scenario, the \elastras\ design can still provide \emph{elasticity} and \emph{scalability} by dynamic partition reassignment based on the load on the system, while providing serializable transactional guarantees within a partition. Additionally, for applications where the designer does not want to statically partition the database, \elastras\ can dynamically partition the database. In addition to \emph{single-object} transactions, \elastras\ can be easily extended to support \emph{minitransactions} as defined by the Sinfonia system~\cite{sinfonia}, but flexible transactions are not supported in the interest of scalability and elasticity. Based on these requirements of modern applications, we are in the process of formalizing the various forms of transactions that can be efficiently executed by \elastras, while having minimal impact of application design and preserving the 3-tier architecture of \emph{web-servers}, \emph{application servers}, with \elastras\ replacing the \emph{database servers} in the cloud, thus providing a high degree of \emph{elasticity} and \emph{flexibility} throughout the entire architecture.

\cut{
\subsection{Challenges in Supporting Online Analysis}
%\noindent \textit{B. Challenges in Supporting Online Analysis}

In addition to providing transactional access, the \elastras\ design can be used to efficiently answer a range of analysis queries aiding online analysis. Since the HTMs cache contains parts of the database, a lot of these read-only queries can be satisfied by an HTM, and this significantly reduces the load on the OTMs. For queries that span a large portion of the database, the cache in an HTM might not be big enough to answer them, and in such a case, a divide-and-conquer approach is used. The query is partitioned and shipped to the appropriate OTMs, where the queries are executed, and the results are transmitted back to the HTM, which aggregates the results and returns them to the application. The efficiency of query execution in the OTMs can be improved by using multi-version concurrency control such as serializable snapshot isolation~\cite{cahill08}. In this paper, we did not discuss indexes and views, and the efficient asynchronous maintenance of these auxiliary structures to enhance analysis. This an important research problem for future work.

%\cut{
\subsection{Cost vs. Performance tradeoff}

There are two types of costs associated with the operations of \elastras\ in the cloud: \emph{first}, the storage cost of the data, and \emph{second}, the compute cost for running the different components of the system. To reduce the cost of operation, an HTM and an OTM can share the same machine instance, but this definitely would have an impact on the performance of the system. Similarly, the \emph{metatdata manager} also adds to the cost of operation. But \elastras\ is designed to access the \emph{metadata manager} only for the critical operations of system maintenance, hence the \emph{metadata}  manager is expected to be lightly loaded, and can be shared across multiple \elastras\ instances. Therefore, it is evident that \elastras\ opens up new avenues for cost vs. performance tradeoffs, and also provides different knobs that allow these metrics to be tuned to suit the application requirements.
}


%\vspace*{0.1in}
%\noindent \textbf{Acknowledgements}
\subsection*{Acknowledgements}

The authors would like to thank the anonymous reviewers for their useful comments and suggestions that helped improve this paper. This work is partly supported by NSF Grants IIS-0744539 and CNS-0423336 

==> evaluation.tex <==
\section{Evaluation Plan}
\label{sec:evaluation}

In this section, we provide a scheme for evaluation and benchmarking for the design suggested in the previous section. Benchmarking of the system is extremely critical for understanding various aspects of the system for different types of workloads. In addition to individual benchmarking, performance comparison with similar systems is also very important. Two closest rivals for \elastras\ are MySQL (traditional database) and SimpleDB (\emph{key-value} store). In this section, we chalk out a scheme for a fair performance comparison with each of these systems, keeping in mind that all the three systems (MySQL, SimpleDB, and \elastras) have been built to achieve different goals.

\subsection{Benchmarking \elastras}

\subsection{Comparison with MySQL}

For transactional workload, in terms of latency, and throughput.

\subsection{Comparison with Amazon SimpleDB} 

For queries in terms of latency and throughput.

==> implementation.tex <==
\section{Implementation Sketch}
\label{sec:implementation}

%In this section, we provide a high level scheme for implementing the proposed design using the cloud interface provided by Amazon Web Services (AWS).

%\noindent \textit{A. Transaction Management in an OTM}

\subsection{Transaction Management}
\label{sec:transaction_mgmt}

In a \emph{statically partitioned} setup, applications can limit transactions to single partitions. Within a partition, \elastras\ provides ACID guarantees similar to transactions in databases. The only subtle difference is in the level of consistency (the C in ACID) guaranteed by \elastras. To obviate distributed synchronization, and minimize the impact of a single TM failure on the operation of the remaining TMs, \elastras\ guarantees consistency only within a partition of the database and there is no notion of consistency \emph{across} partitions or global serializability~\cite{weikum}. Efficient performance can therefore be achieved since an OTM is guaranteed exclusive access to the partitions it \emph{owns}, and proven techniques for concurrency control, isolation, and recovery in traditional databases~\cite{weikum,jim_gray_book} can be used in designing the OTM. Since an OTM has exclusive access to the partition, it can aggressively cache the database contents in its local disk, and the updates can be asynchronously applied to the distributed store in a manner similar to database checkpointing~\cite{weikum}. Since \emph{dynamic partitioning} does not allow applications to limit transactions to a single partition, \elastras\ only supports \emph{minitransactions}~\cite{sinfonia} in this setup, while supporting both forms of transactions for a \emph{statically partitioned} setup. In executing a \emph{minitransaction}, there is no need for synchronization amongts participating OTMs, and hence, \emph{minitransactions} can be efficiently executed within \elastras.

%\noindent \textit{B. Recovery done right}

\subsection{Recovery done right}
\label{sec:recovery}
%\textit{$1)$ Failure of OTM:}
%\subsubsection{Failure of OTM}
\noindent \textbf{Failure of OTM:}
To ensure the durability of transactions, OTMs use write-ahead logging. As a result, techniques such as ARIES ~\cite{mohan91_aries_rrh} and other similar recovery techniques~\cite{weikum,jim_gray_book} can be used for efficient recovery. In the AWS model, when a machine instance crashes, its local disk is also lost. Therefore, to guarantee the durability and persistence of transactions beyond the failure of an OTM, the log entries of committed transactions should be stored on some persistent storage. But since logging must be performed during normal transaction execution, the performance of an OTM would suffer if the log entries are \emph{forced} to a distributed store like S3. AWS provides a better solution in the form of Elastic Block Storage (EBS), which provides persistence beyond instance failures, allowing log entries to be stored on EBS. Our initial experiments with EBS showed that for sequential reads and writes, the performance of EBS is comparable to disks associated with AWS machine instances. Therefore, using EBS for both caching data pages, and storing logs would provide better performance, though at a higher dollar cost. When an OTM fails, its lease with the \emph{metadata manager} expires, and once the \emph{master} notices that the OTM instance has failed, it can instantiate a new OTM, which recovers the state of the failed OTM from the logs. A similar mechanism is used in Bigtable~\cite{bigtable} to deal with \emph{tablet server} failures.

%\textit{$2)$ Failure of HTM:}
%\subsubsection{Failure of HTM}
\noindent \textbf{Failure of HTM:}
Very little state is associated with the HTMs and hence, handling HTM failures is easier. All progress of a read-only transaction is lost when the HTM executing it fails. Clients of such transactions time out, and application specific recovery triggered. For \emph{minitransactions}~\cite{sinfonia}, no state is associated with the \emph{coordinator}, and hence the recovery principles described in Sinfonia~\cite{sinfonia} can be used to recover a \emph{minitransaction} from HTM or \emph{coordinator} failures.

\cut{
\subsubsection{Failures in the data storage layer}
%\textit{$3)$ Failures in the data storage layer:}
The \emph{distributed data storage layer} provides the abstraction of a fault-tolerant storage, and hence failures inside S3 are transparent to the system. In addition, since the OTMs can aggressively cache the data of the partitions, even if certain portions of S3 are not available, if the OTM is operational, it can continue to serve the partition out of its cache without any visible impact on system performance.
}

%\noindent \textit{C. Elasticity}

\subsection{Elasticity}
\label{sec:elasticity}

The ability of the system to deal with dynamic partition reassignments is the basis for the \emph{elasticity} of the data store. When the load on the system is low, the system can operate with a small number of HTM and OTM instances. As the load on the system increases, the partitions can be reassigned to lesser loaded OTMs, or new OTMs can be spawned to absorb the load and take ownership of some partitions from the heavily loaded transaction managers. Since the HTMs do not share any state information, spawning new HTMs is easy, and amounts to spawning new instances that can immediately start absorbing the load. On the other hand, when a new OTM instance is created, it has to acquire a lease from the \emph{metadata manager}, obtain control for some of the partitions, update the \emph{metadata} to reflect the modified mapping, and perform any partition specific recovery. Once this is done, the new OTM is ready to execute transactions for the partition, while the old OTMs reject or redirect transactions of the reassigned partitions. Similarly, when the load decreases, the system can detect this and decide to remove OTM and/or HTM instances. Removal of HTM instances requires notifying the load balancer about the update, and then stopping the physical instance. Removing OTM instances requires updates to the \emph{metadata} and the transfer of control of the partitions to some other OTM. Once control is transferred, the physical OTM instance can be stopped. Since AWS uses a \emph{pay-as-you-go} model, stopped instances do not incur any cost, and hence, at low loads, the cost of operating the data store also reduces. 

==> related.tex <==
\section{Related Work}
\label{sec:related}

%Over the last two or three decades, a lot of effort has gone into scaling out the database servers, as the amount of data being managed, and the number of transactions keep on increasing. The original attempt was to design distributed databases, such as R$^*$~\cite{linday-rstar84}, where the database would scale out to a distributed system of nodes. The noble aim was that the application would still be provided the abstraction of a centralized database, and the underlying database server would tackle the complexity of distribution of data and control. But the overhead for distributed synchronization, atomic commitment, and recovery in a distributed setting was extremely high, and as a result, these systems were not widely used. Instead, database partitioning and various other ad-hoc techniques were used for scaling out large database systems. But the semantics of the partitioned databases are somewhat different from that on a single node.

Based on the expertise gained from building distributed database systems~\cite{linday-rstar84,ssd1-benstein}, researchers and designers have realized that supporting distributed transactions does not allow scalable and available designs. Hence, to satisfy the scalability requirements of web applications, designers have sacrificed the ability to support distributed transactions~\cite{helland07cidr}. This resulted in the design of simpler data stores based on the \emph{key-value} schema, where tables are viewed as a huge collection of \emph{key-value} entries, and the values might have some structure, or may be viewed as uninterpreted strings of bytes~\cite{das08c}. Examples of these systems include Bigtable~\cite{bigtable}, Dynamo~\cite{dynamo}, PNUTS~\cite{pnuts}, Amazon SimpleDB, Facebook Cassandra, and many more. These systems limit access granularity to single key accesses, while providing minimal consistency and atomicity guarantees on multi-key accesses. This allows the system to horizontally partition the tables, without worrying about the need for distributed synchronization. These systems can be viewed to be the other end of the spectrum of data management solutions when compared to transactional databases. In particular, these systems are designed for high scalability and availability, but not to replace the traditional databases for consistent transactional properties, and recovery.

Other systems spanning the middle ground include Sinfonia~\cite{sinfonia}, where the \emph{minitransaction} primitive demonstrates that distributed transactions and distributed commitment, if used in a prudent manner, can be used for the design of scalable distributed systems. Similarly, Chubby~\cite{chubby}, which uses the expensive Paxos consensus protocol~\cite{paxos}, forms the core of scalable data management systems such as Google File System~\cite{gfs} and Bigtable~\cite{bigtable}. These systems demonstrate that even though the paradigm of distributed databases was not successful, a lot of important concepts that were developed for these systems can be effectively used in modern scalable systems. %However, the way such techniques are used in these systems, and the design choices these systems eschew make them interesting. In this paper, we design our system based on the lessons gleaned from such systems.

There have been efforts in designing databases for the cloud. Brantner et~al~\cite{brantner08_s3} suggest a design for a database server that can use Amazon's S3 as a storage layer for the database engine, while the transaction manager might be located inside or outside the cloud. On the other hand, Lomet et~al.~\cite{lomet09_cidr} suggest a radically different approach where they suggest unbundling the transaction and the data manager. Even though these techniques open many interesting research avenues, the authors do not address the problem of elastic scaling of database systems in the cloud. \elastras\ has been designed with the goal of \emph{scalable} and \emph{elastic} transaction management in the cloud. 
